Experiments on Properties of Hidden Structures of Sparse Neural Networks

Sparsity in the structure of Neural Networks can lead to less energy consumption, less memory usage, faster computation times on convenient hardware, and automated machine learning. If sparsity gives rise to certain kinds of structure, it can explain automatically obtained features during learning. We provide insights into experiments in which we show how sparsity can be achieved through prior initialization, pruning, and during learning, and answer questions on the relationship between the structure of Neural Networks and their performance. This includes the first work of inducing priors from network theory into Recurrent Neural Networks and an architectural performance prediction during a Neural Architecture Search. Within our experiments, we show how magnitude class blinded pruning achieves 97.5% on MNIST with 80% compression and re-training, which is 0.5 points more than without compression, that magnitude class uniform pruning is significantly inferior to it and how a genetic search enhanced with performance prediction achieves 82.4% on CIFAR10. Further, performance prediction for Recurrent Networks learning the Reber grammar shows an $R^2$ of up to 0.81 given only structural information.

==> content/broader-impact.tex <==
\section*{Broader Impact}

% TODO
-

%Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
%Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
%who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
%biases in the data. If authors believe this is not applicable to them, authors can simply state this.



==> content/discussion.tex <==
\section{Discussion}\label{sec:discussion}

We compared five pruning techniques for pruning feed-forward networks, namely random pruning, magnitude class blinded, magnitude class uniform, magnitude class distributed, and optimal brain damage. 
Out of these five, random pruning immediately showed an accuracy drop, while the other four performed consistently near original performance for over 60\% compression rate. 
In the end, magnitude class blinded outperformed the remaining four.

While applying pruning on recurrent networks, we found models to perform consistently better for up to 60\% pruning. 
All the pruned models regain the original performance in just one to two epochs of re-training. 
This means these recurrent networks can achieve the same results as any dense recurrent network with almost 60\% fewer weights. 
As opposed to our expectations, LSTM and GRU recovered even after 100\% pruning of hidden-to-hidden weights. 
In LSTM, this might be due to a separate cell state that acts as long-term memory.

Our experiment with random structural priors for recurrent networks aimed to find essential graph properties and use them for performance prediction. 
Similar to the results of the paper, three of the essential features are the number of edges, vertices, and source nodes. 
Although the construction and properties of Watts–Strogatz, and Barabási–Albert random graphs are different, recurrent networks based on this two performed equally with RNN\_Tanh and RNN\_ReLU. 
Barabási–Albert based recurrent networks perform better than Watts–Strogatz based with LSTM and GRU.

